Off-Policy Imitation Learning from Observations

Learning from Observations (LfO) is a practical reinforcement learning scenario from which many applications can benefit through the reuse of incomplete resources. Compared to conventional imitation learning (IL), LfO is more challenging because of the lack of expert action guidance. In both conventional IL and LfO, distribution matching is at the heart of their foundation. Traditional distribution matching approaches are sample-costly which depend on on-policy transitions for policy learning. Towards sample-efficiency, some off-policy solutions have been proposed, which, however, either lack comprehensive theoretical justifications or depend on the guidance of expert actions. In this work, we propose a sample-efficient LfO approach that enables off-policy optimization in a principled manner. To further accelerate the learning procedure, we regulate the policy update with an inverse action model, which assists distribution matching from the perspective of mode-covering. Extensive empirical results on challenging locomotion tasks indicate that our approach is comparable with state-of-the-art in terms of both sample-efficiency and asymptotic performance.

==> sections/bc_reg_backup.tex <==

\subsection{Inverse Model Regularization} 
We find it helpful to further enforce an inverse dynamic constraint when learning policy $\pi$. 
%Specifically, we learn an inverse model $\PI$ based on samples from distribution $\muR$. 
Given arbitrary transition $s \to s'$, an inverse model $\PI$ should yield a distribution of actions that maximize the probability of seeing this transition in the given MDP: 
\begin{align} \label{eq:inverse}
\forall (s, s') \sim \cS \times \cA,  
\PI^* = \arg \max_{\PI: \cS \times \cS \to \cA} \int_{\cA} \PI(a|s,s') \cP(s'|s,a) da 
\end{align}  

{\remark When the environment is deterministic and bijective, the inverse dynamics probability is also deterministic, and is policy-agnostic.}
We defer proof into the appendix. 

When the MDP is stochastic, an inverse-model is not guaranteed to recover the expert action. However, we prove that it is still worthwhile to enforce the inverse model constraints, as it minimizes a conditional $\KL$-divergence on \textit{forward state transition distributions} between $\mut$ and $\mupi$: 
\begin{align*}
    %\arg \min_\pi
    &\cD_\KL[\mut(s'|s) || \mupi(s'|s)] := \int_{\cS \times   \cS} \mut(s) \mut(s'|s) \log \frac{\mut(s’|s) }{\mupi(s’|s) } ds ds' \\
    &= \int_{\cS \times   \cS} \mut(s) \mut(s'|s) \log  \mut(s’|s) ds ds' -  \int_{\cS \times   \cS} \mut(s) \mut(s'|s) \log  \mupi(s’|s) ds ds'  \\
    &= \underbrace{-H(\mut(s'|s))}_{\text{not optimizable~} \wrt \pi} -  \int_{\cS \times   \cS} \mut(s,s')  \log  \mupi(s’|s) ds ds' \\
    &= -H(\mut(s'|s))   -  \int_{\cS \times   \cS} \mut(s,s')  \log  \int_{\cA} \pi(a|s) \cP(s'|s,a) da ds ds' \\
    %&\leq -H(\mut(s'|s))   -  \int_{\cS \times   \cS} \mut(s,s') \int_{\cA}  \underbrace{\log \big(  \pi(a|s) \cP(s'|s,a) }_{\text{{Jensen's inequality}}} \big) da ds ds' \\
    &\geq -H(\mut(s'|s))   -  \int_{\cS \times   \cS} \mut(s,s')    \log \int_{\cA}  \underbrace{   \PI^*(a|s,s') \cP(s'|s,a) }_{\text{ \eq{ \ref{eq:inverse} } }}   da ds ds' 
\end{align*} 


where we define $\mupi(s’|s)= \int_\cA \pi(a|s) \cP(s'|s,a) da$, and the same for $\mut(s’|s)$ .
$\cD_\KL[\mut(s'|s) || \mupi(s'|s)] $ is minimized when $\pi(\cdot|s) = \PI^*(\cdot|s,s') ~ \forall s, s \sim \mut(s,s')$. 
Intuitively, this constraint can be considered as performing \textit{mode covering}, while the main objective is performing \textit{mode seeking}.
% \begin{align*}
%     \max\pi \JINV(\pi) &= - \cE_{s,s' \sim \mut(\cdot|s), a \sim \PI^*(\cdot|s,s')} [\log \pi(a|s)] \\
%     &= - \int_{\cS \times \cS} \mut(s,s') \int_{\cA} \PI^*(a|s,s') \log \pi(a|s) da ds ds'
% \end{align*}


% {\assumption the inverse model is Multi-variant Gaussian, with it mean depending on the state-transition:
% \begin{align*}
%     &\PI(\cdot |s, s') \sim \cN(\mu(s,s'), \mathbf{\Sigma} ),\\
%     \forall a \sim \cA, \log &\PI(a|s,s') \propto - ||\mu(s,s') - a||_2
% \end{align*}
% }



 

==> sections/condKL.tex <==
\section{Bring the Gap between LfO and LfD } \label{sec:condKL}
\judycom{TBD.} Approaches should minimize the conditional KL-divergence specified in \eq{\ref{eq:gap1}} (or \eq{\ref{eq:gap2}}) or its lower-bound.

==> sections/dice_discuss.tex <==

\subsection{Dilemma of Off-Policy Distribution Matching Given Only Expert Observations} \label{sec:dice-dilemma}

% A crucial limitation of most IL approaches relies in their on-policy sampling to approximate the expectation on distribution $\mupi(s,a)$, which is highly sample-inefficient.
% %
A solution to this issue is to apply the idea of distribution correction estimation (DICE) \cite{nachum2019dualdice,zhang2020gendice} to enable off-policy distribution matching, as realized by ValueDICE \cite{kostrikov2019imitation}.

The rationale behind ValueDICE \cite{kostrikov2019imitation} is to transform the IL Objective in \eq{\ref{obj:dice}} into its variational form, which eliminates the need of \textit{on-policy} expectations.
%They observe that an optimal $x$ learned by optimizing \eq{\ref{obj:dice}} is just the density ratio between two distributions: $x^*(s,a) = \frac{\mupi(s,a)}{\mut(s,a)}$.
%
To achieve this goal, the change-of-variables technique \cite{nachum2019dualdice} is applied to learn a \textit{state-action} function $Q: \cS \times \cA \to \RR$ derived from $x(s,a)$. This $Q$ function is a fixed point to an Bellman Equation \cite{kirk1970optimal}:
\begin{small}
   \begin{align*}
   Q(s,a):=  x(s,a) + \gamma \cE_{s' \sim \cP(.|s,a), a'\sim \pi(.|s')}[Q(s',a')] = x(s,a) + \cB^\pi Q(s,a) .
   \end{align*} 
\end{small}
After applying change-of-variables with $x(s,a)= (Q - \cB^\pi Q)(s,a)$, and a series of telescoping, \eq{\ref{obj:dice}} can be equivalently transformed into the following off-policy objective:
\begin{small}
   \begin{align}
   %&\max_\pi \min_{x: \cS \times \cA \to \RR} \cE_{(s,a)\sim d^\pi}[- x(s,a)] +  \cE_{(s,a) \sim \mut}[f_*(x(s,a))]  \nonumber \\
   %\equiv &\max_\pi \min_{v: \cS \times \cA \to \RR} \cE_{(s,a)\sim d^\pi}[-(v- \cB^\pi v)(s,a)] +  E_{(s,a) \sim \mut}[f_*((v- \cB^\pi v)(s,a))]  \nonumber \\ 
   %\equiv &\max_\pi \min_{v: \cS \times \cA \to \RR} -(1 - \gamma)\cE_{s_0 \sim p_0, a_0 \sim \pi(\cdot|s_0)}[Q(s,a)] +  E_{(s,a) \sim \mut}[f_*((v- \cB^\pi v)(s,a))]  \label{obj:dice-reduce}
   \max_\pi \min_{v: \cS \times \cA \to \RR} -(1 - \gamma)\cE_{s_0 \sim p_0, a_0 \sim \pi(\cdot|s_0)}[Q(s,a)] +  \cE_{(s,a) \sim \mut}[f_*((Q- \cB^\pi Q)(s,a))]  \label{obj:dice-reduce}
   \end{align} 
   \vskip -0.1in
\end{small}

The above objective eliminates the dependence on distribution $\mupi(s,a)$ and can be optimized with off-policy learning.
%
This strategy, however, is not directly applicable to a ILfO scenario, as learning the $Q$ function is unfeasible without knowing expert actions.
%

Alternatively, if we follow the similar idea and consider the dual form of an ILfO objective:
\begin{small}
   \begin{align*}
   \max_\pi - \cD_f[\mupi(s,s')||\mut(s,s')] \equiv \max_\pi \min_{x: \cS \times \cS \to \RR} \cE_{(s,s')\sim d^\pi}[- x(s,s')] +  \cE_{(s,s') \sim \mut}[f_*(x(s,s'))],
   \end{align*} 
   \vskip -0.1in
\end{small}
and learn a \textit{value} function dependent only on \textit{states}: 
\begin{align*}
   v(s,s'):= x(s,s') + \cB^\pi v(s,s') = x(s,s') + \gamma \cE_{ a'\sim \pi(.|s'),s'' \sim \cP(.|s',a') }[v(s',s'')],
\end{align*}  
Then we can equivalently transform the ILfO objective of \eq{\ref{obj:dice-lfo}} into the following:
\begin{small}
\begin{align} %\label{obj:dice-lfo}
  \max_\pi \min_{v: \cS \times \cS \to \RR} - (1 - \gamma) \underbrace{\cE_{s_0 \sim p_0, s_1 \sim \cP(\cdot|s_0, \pi(s_0))}}_{\text{term 1}} [v(s_0, s_1)] +  \underbrace{E_{(s,s') \sim \mut}[f_*( (v - \cB^\pi v)(s,s'))] }_{\text{term 2}}.  \nonumber
\end{align}
\vskip -0.1in
\end{small}
However, this objective is still difficult to optimize, due to a troublesome bellman operator in term 2, $\cB^\pi v(s,s') = \gamma \cE_{ a'\sim \pi(.|s'),s'' \sim \cP(.|s',a') }[v(s',s'')]$,
as it requires the knowledge of $\cP(\cdot|s, \pi(s) ), ~ \forall s \sim \mut(s)$. In another word, for any state sampled from the \textit{expert} distribution, we need to know what would be the next state if following  policy $\pi$ from this state.
%
A similar issue occurs in term 1, where $s_1$ is sampled from $\cP(\cdot|s_0, \pi(s_0)).$
%
Consequently, in an ILfO problem setting, directly applying the DICE principle to minimize $\cD_f[\mupi(s,s)|| \mut(s,s')]$ loses its advantage, as it incurs a dependence on a forward transition model.
 
In next section, We show how we address sample efficiency by deriving a feasible upper-bound from the original IL objective, which enables \textit{off-policy} optimization in a {principled} manner, and avoids the dilemma of the dependence on a forward-transition model. 

==> sections/experiment-backup.tex <==
% !TEX ROOT=../main.tex

\section{Experiments}
\vskip -0.15in
We compare \opolo against the state-of-the-art LfD and LfO approaches on MuJuCo benchmarks, which are locomotion tasks in continuous state-action space. In accordance with our assumption in Sec~\ref{sec:inverse-action}, these tasks have \textit{deterministic} dynamics. Original rewards are removed from all benchmarks to fit into an IL scenario.
%
For each task, we collect 4 trajectories from an pre-trained expert policy. All illustrated results are evaluated across 5 random seeds. 

We select 4 representative baselines for comparison: \GAIL (on-policy LfD), \DAC (off-policy LfD), \GAIfO (on-policy LfO), and \BCO (off-policy LfO). Among these baselines, \DAC and \GAIL can be considered as oracle references, as we provide them with  both expert \textit{states} and \textit{actions}, while all other approaches only have access to expert \textit{states}.
%
More experimental details can be found in the supplementary material.

Our experiments focus on answering the following important questions:
\begin{enumerate} 
\vskip -0.2in
\item \textit{Asymptotic performance}: Is \opolo able to achieve expert-level performance given a limited number of expert observations? 

\item \textit{Sample efficiency}: Can \opolo recover expert policy using less interactions with the environment, compared with state-of-the-art?

\item \textit{Effects of the inverse action regularization}: Does the inverse action regularization useful in speeding up the imitation learning process? \label{q:inverse-model}  
\end{enumerate} 

\subsection{Performance Comparison}
\vskip -0.1in
\opolo can recover expert performance given a fixed budget of expert observations.
%
As shown in Figure \ref{fig:ep4-comparison}, \opolo reaches (near) optimal performance in all benchmarks. 
%
For simpler tasks such as \textit{Swimmer} and \textit{InvertedPendulum}, most baselines can successfully recover expertise.
%
For other complex tasks with high state-action space, on-policy baselines, such as \GAIL and \textit{GAIfO}, are struggling to reach their asymptotic performance within a limited number of interactions.
%
On the other hand, the off-policy baseline \BCO is easily trapped to sub-optimality due to its behavior cloning-like strategy.
% 
For fair comparison, we summarize the performance of all \textit{off-policy} approaches in Table~\ref{table:offpolicy-comparison}, given a fixed number of interaction steps. 
% 
The asymptotic performance of \opolo is comparable to \textit{DAC}, which enjoys the advantage of off-policy learning and extra action guidance.
%

\begin{small} 
\begin{table}[htb]
    \begin{center}
    \scalebox{0.88}{
    \hskip -0.4 in
    \begin{tabular}{p{1.5cm}p{2.2cm}p{2.1cm}p{2.2cm}p{1.9cm}p{2.1cm}p{2.3cm}p{2cm}}
    %\begin{tabular}{lp{2.5cm}p{2.6cm}p{2.6cm}p{2.5cm}p{2.5cm}p{2.5cm}}
    \hline
    \textbf{Env} & \textbf{HalfCheetah} & \textbf{Hopper} & \multicolumn{1}{c}{\textbf{Walker}} & \multicolumn{1}{c}{\textbf{Swimmer}} & \textbf{Ant} & \hskip -0.2in \textbf{InvertedPendulum} \\ \hline 
    %\GAIfO    & $4213.86\pm306.45$ &  $2999.33\pm599.07$    & $2876.66\pm1303.14$    & $d$  &$2290.27\pm1111.09$  & $486.54\pm108.23$   \\ \hline
    \BCO & 3881.10$\pm$938.81 & 1845.66$\pm$628.41 & 421.24$\pm$135.18 & 256.88$\pm$4.52 & 1529.54$\pm$980.86 & 751.05$\pm$325.16 \\ \hline
    
    %
    \opolox    & \textbf{7632.80$\pm$128.88}  & \textbf{3581.85$\pm$19.08} & 3947.72$\pm$97.88  & 246.62$\pm$1.56  &  5112.04$\pm$321.42   & \textbf{1000.00$\pm$0.00} \\ \hline
    %
    \opolo    & {7336.96}$\pm${117.89} &  {3517.39}$\pm${25.16}    & {3803.00}$\pm${979.85}    & \textbf{257.38$\pm$4.28}  & \textbf{5783.57}$\pm$\textbf{651.98}  & \textbf{1000.00$\pm$0.00}  \\ \hline
    %
    \DAC    & 6900.00$\pm$131.24 &  {3534.42$\pm$10.27}    &  \textbf{4131.05$\pm$174.13}    & 232.12$\pm$2.04  &5424.28$\pm$594.82  &  \textbf{1000.00$\pm$0.00} \\ \hline
    %
    Expert    & 7561.78$\pm$181.41 &  3589.88$\pm$2.43 & 3752.67$\pm$192.80    & 259.52$\pm$1.92  & 5544.65$\pm$76.11 & 1000.00$\pm$0.00  \\ \hline
    $(\cS,\cA)$    & $(17,6)$ &  $(11,3)$ & $(17,6))$    & $(8,2)$  & $(111,8)$ & $(4,1)$  \\ \hline
    \end{tabular}}
    \end{center}
    \caption{Evaluated performance of \textit{off-policy} approaches. Results are averaged over 50 trajectories. }
    \label{table:offpolicy-comparison}
    \vskip -0.2in
    \end{table} 
\end{small} 


\subsection{Sample Efficiency}
\vskip -0.1in
\opolo is comparable to and sometimes superior than \textit{DAC} in all evaluated tasks, and is much more sample-efficient than other baselines. 
%
As show in Figure~\ref{fig:ep4-comparison},
\opolo is significantly more efficient than on-policy approaches.
%
The sample-efficiency of \opolo is emphasized by benchmarks with high state-action dimensions. 
%We summarize the state-action dimension of each benchmark in Table \ref{table:offpolicy-comparison}.
%
In particular, for tasks such as \textit{Ant} or \textit{HalfCheetah}, the performance curves of \textit{on-policy} baselines are barely improved at early learning stages. One intuition is that they need more explorations to build the current support of the learning policy, which cannot benefit from cached transitions.
%
For these challenging tasks, \opolo is even more sample-efficient than \textit{DAC} that has the guidance of expert actions. We ascribe this improvement to the \textit{mode-covering} regularization of \textit{OPOLO}, whose effect will be further analyzed in Sec~\ref{sec:ab-study}.
%
Meanwhile, another off-policy approach \BCO is prone to overfitting and performance degradation (see \textit{InvertedPendulum} and \textit{HalfCheetah}), which indicates that pursuing the effect of \textit{mode covering} alone is not sufficient to recover expertise.
%

\subsection{Ablation Study} \label{sec:ab-study}
\vskip -0.05in
In this section, we further analyze the effects of the inverse action regularization by a group of ablation studies.
%
Especially, we implement a variant of \opolo that does not learn an inverse action model to regulate the policy update. We compare this approach, dubbed as \opolox, against our original approach as well as the \DAC algorithm. 

\textit{\textbf{Effects on Sample efficiency:}} Performance curves in Figure~\ref{fig:ep4-ab} show that removing the inverse action regularization from \opolo slightly affects its sample-efficiency, although the degraded version is still comparable to \textit{DAC}. 
%
This impact is more visible in challenging tasks such as \textit{HalfCheetah} and \textit{Ant}.
%
From another perspective, the same phenomenon indicates that an inverse action regularization is beneficial for accelerating the IL process, especially for games with high observation-space.
%
An intuitive exploration is that, while our main objective serves as a driving force for \textit{mode-seeking}, a regularization term assists by encouraging the policy to perform \textit{mode-covering}. Combing these two motivations leads to a more efficient learning strategy.
%  

\textit{\textbf{Effects on Performance:}}
Given a reasonable number of transition steps, the effects of an inverse-action model are less obvious regarding the asymptotic performance. As shown in Table~\ref{table:offpolicy-comparison}, \opolox~is mostly comparable to \opolo and \textit{DAC}. 
%
This implies that the effect of the \textit{state-covering} regularization will gradually fade out once the policy learns a reasonable state distribution. 
%
In fact, \opolox~even achieves highest scores in 2 out of 6 benchmarks with a small margin. 
%
From another perspective, it indicates that following our main objective alone is sufficient to recover expertise. 
%
Comparing with \BCO which uses the inverse model solely for behavior cloning, we find it more effective when serving as a regularization to assist distribution matching from a \textit{forward} direction.

\vskip -0.1in
\begin{figure*}[ht]  
    %\vskip -0.1in
    \begin{center}
        \hskip -0.4in %\qquad 
        \begin{minipage}[b]{.33\textwidth}
        %\begin{minipage}[b]{.33\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Swimmer-v2-ep4-explore.pdf}}  
        \end{minipage} 
        \hskip -0.05in %\qquad 
        \begin{minipage}[b]{.33\textwidth} 
            \centerline{\includegraphics[width=\columnwidth]{figs/InvertedPendulum-v2-ep4-explore.pdf}} 
        \end{minipage}  
        \begin{minipage}[b]{.33\textwidth} 
            \centerline{\includegraphics[width=\columnwidth]{figs/HalfCheetah-v2-ep4-explore.pdf}} 
        \end{minipage} %\hskip -0.2in  
        
        \hskip -0.3in %\qquad 
        \begin{minipage}[b]{.35\columnwidth} 
            \centerline{\includegraphics[width=\columnwidth]{figs/Walker2d-v2-ep4-explore.pdf}} 
        \end{minipage} 
        \hskip -0.05in 
        \begin{minipage}[b]{.34\columnwidth} 
            \centerline{\includegraphics[width=\columnwidth]{figs/Ant-v2-ep4-explore.pdf}} 
        \end{minipage} 
        \hskip -0.05in 
        \begin{minipage}[b]{.34\columnwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Hopper-v2-ep4-explore.pdf}} 
        \end{minipage} 
    \caption{Interaction steps ($x$-axis) versus learning performance ($y$-axis). \opolo  is the most sample-efficient to reach expert-level performance (Grey horizontal line). }
    \label{fig:ep4-comparison}
    \end{center}
    \vskip -0.1in
 \end{figure*}

\vskip -0.15in
\begin{figure*}[ht]  
    %\vskip -0.1in
    \begin{center}
        \hskip -0.4in %\qquad 
        \begin{minipage}[b]{.33\columnwidth}
        %\begin{minipage}[b]{.33\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Swimmer-v2-ep4-ablation.pdf}}  
        \end{minipage} 
        %\hskip -0.05in %\qquad 
        \begin{minipage}[b]{.33\columnwidth}
        %\begin{minipage}[b]{.33\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/InvertedPendulum-v2-ep4-ablation.pdf}} 
        \end{minipage} %\hskip -0.3in
       % \hskip -0.05in %\qquad 
        \begin{minipage}[b]{.34\columnwidth}
        %\begin{minipage}[b]{.33\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/HalfCheetah-v2-ep4-ablation.pdf}} 
        \end{minipage} %\hskip -0.2in 
        %
        
        \hskip -0.3in  
        \begin{minipage}[b]{.35\textwidth}
        %\begin{minipage}[b]{.33\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Walker2d-v2-ep4-ablation.pdf}} 
        \end{minipage} 
        \hskip -0.05in  
        \begin{minipage}[b]{.34\textwidth}
        %\begin{minipage}[b]{.33\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Ant-v2-ep4-ablation.pdf}} 
        \end{minipage}   
        \hskip -0.05in  
        \begin{minipage}[b]{.34\textwidth}
        %\begin{minipage}[b]{.33\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Hopper-v2-ep4-ablation.pdf}} 
        \end{minipage} 
    \vskip -0.1in
    \caption{Removing the inverse action regularization (\opolox) results in slight efficiency drop, although its performance is still comparable to \opolo and \textit{DAC}.}
    \label{fig:ep4-ab}
    \end{center}
    \vskip -0.1in
 \end{figure*}


==> sections/gaps.tex <==
\section{Gaps Between LfO and IL}
% First, we would like to specify two naive Learning-from-Observation (LfO) objectives:

% \textbf{Naive LfO} on single states: 
%    \begin{align} \label{eq:lfo1}
%       \min_\pi \KL(\dpi(s)||\dt(s))
%    \end{align}

% \textbf{LfO} on state transitions: 
%    \begin{align} \label{eq:lfo2}
%       \min_\pi \KL(\dpi(s,s')||\dt(s,s'))
%    \end{align}

% Both of them have a gap to fix in order to reach the Learning-from-Demonstration (LfD) objective \cite{yang2019imitation}:

% \textbf{LfD:}
% \begin{align} \label{eq:lfd}
%    \min_\pi \KL(\dpi(s,a,s')||\dt(s,a,s')):= \KL(\dpi(s,a)||\dt(s,a))
% \end{align}

% \cite{yang2019imitation} states the connection between LfO and LfD:
% \begin{align} \label{eq:gap1}
%    \KL(\dpi(s,a) || \dt(s,a)) = \cD_\KL(\dpi(a|s,s')||\dt(a|s,s')) + \KL(\dpi(s,s') || \dt(s,s')). 
% \end{align}
% where $\cD_\KL$ denotes \textit{conditional} KL-Divergence. Similarly, we can derive at the following connection:
We begin with following property:


%A surrogate solution is to learn from teacher observations with objectives of either \eq{\ref{eq:lfo1}} or \eq{\ref{eq:lfo2}}, and bring the gap between the surrogate and the primal in the meantime.

%In Section \ref{sec:OPEDICE} , we propose efficient solutions to LfO, inspired by the off-policy-estimation ideas from the DICE family \cite{zhang2020gendice,nachum2019dualdice,kostrikov2019imitation}. Our solutions are applicable to both objectives of \eq{\ref{eq:lfo1}} and \eq{\ref{eq:lfo2}}.

%In Section \ref{sec:condKL}, we discuss how to address the gaps listed in \eq{\ref{eq:gap1}} and \eq{\ref{eq:gap2}} \judycom{(TBD)}. 

==> sections/wdice.tex <==
\section{Approach 3: Imitation Learning by Wasserstein-DICE with Estimated Actions}
\subsection{Wasserstein-DICE}
The Wasserstein-1 Distance of $\mupi$ and $\mut$ can be estimated by learning its dual form:
\begin{align*}
    \Dw (\mupi, \mut) = \sup_{D: \cS \times \cA \to \dR, D \in \dD} \cE_{(s,a) \sim \mut}[D(s,a)] - \cE_{ (s,a) \sim \mupi} [D(s,a)]
\end{align*}

where $\dD$ is the set of 1-Lipschitz functions:
\begin{align*}
    ||D||_L \leq 1 ~~\forall D \in \dD 
\end{align*} 

{\remark
An optimal $\pi$ that minimizes the Wasserstein-1 Distance between $\mupi$ and $\mut$ is the saddle-point solution to the following min-max problem:
\begin{align} 
    \min_\pi \max_{D \in \dD} \cE_{(s,a) \sim \mut}[D(s,a)] - \cE_{(s,a) \sim \mupi} [D(s,a)] \label{obj:wdice}
\end{align}
}

By leveraging the change-of-variables technique \cite{nachum2019dualdice}, we can re-write the objective in \eq{\ref{obj:wdice}} as follows:
\begin{align*}
    \min_\pi \max_{ ||Q||_L \leq 1} \cE_{(s,a) \sim \mut}[(Q - B^\pi Q) (s,a)] - \cE_{(s,a) \sim \mupi} [ (Q - B^\pi Q) (s,a) ]  
\end{align*}

where $(Q - B^\pi Q)(s,a) = Q(s,a) - \gamma \cE_{s' \sim \cP(\cdot|s,a), a' \sim \pi(\cdot |s')}[Q(s',a')] \text{,~with~} \gamma \in (0,1].$

{ \remark  
For arbitrary $Q$ function, if $Q$ is 1-Lipschitz function, then $Q- B^\pi Q $ is also 1-Lipschitz \judycom{(Not verified yet)}.}

By further applying a chain-rule, we reach at the following equivalent objective:
\begin{align*}
    \min_\pi \max_{ ||Q||_L \leq 1} \cE_{(s,a) \sim \mut}[(Q - B^\pi Q) (s,a)] - \cE_{s_0 \sim p_0, a_0 \sim \pi } [ Q (s_0,a_0) ] 
\end{align*} 
In practice, we use the gradient penalty proposed \cite{gulrajani2017improved} to enforce the Lipschitz constraint on $Q$.  

\subsection{Switch from LfO to LfD by Inferring Missing Actions}
A remaining challenge is that we do not have expert labels. \judycom{A strawman solution would be learning an inverse model to infer the missing expert action labels, and reduce the LfO problem to LfD.}

Primal Objective:
\begin{align*}
  \theta^* = \arg \min_\theta  J_\pi(M, \RE; \pi) &:= \Dw (\mupi(s,a), \mut(s,a))
\end{align*}

Surrogate Objective: we alternatively learn $\pi$ and $M$ with the following objectives:
\begin{itemize}
   \item 
Update $M$:
\begin{align*}
   \varphi^* = \arg \min_\varphi J_M(\RB;\varphi) := \cE_{(s,a,s') \sim \RB} \big[ ||M_\varphi(s,s') - a ||^2_2  \big]
\end{align*}
 
\item Update $\pi$ and $Q$ by optimizing the min-max objective with inferred actions:
\begin{align} \label{obj:dual-wdice}
\min_\pi \max_{ ||Q||_L \leq 1} \cE_{(s,s'\cdot) \sim \mut(s,s')}[(Q - B^\pi Q) (s, M_\varphi(s,s'))] - \cE_{s_0 \sim p_0, a_0 \sim \pi } [ Q (s_0,a_0) ] 
\end{align}
\end{itemize}

\section{Approach 3:  Wasserstein-DICE on State-Only Distributions}
Similar to \eq{\ref{obj:wdice}}, we can minimize Wasserstein-1 Distance on $\mupi(s)$ and $\mut(s)$ by learning $\pi$ and $D$ to optimize the following objective:
\begin{align}
    \min_\pi \max_{|D|_L \leq 1} \cE_{(s) \sim \mut}[D(s)] - \cE_{(s) \sim \mupi} [D(s)] \label{obj:wdice-state}
\end{align}

As mentioned in Section \ref{sec:OPEDICE}, a challenging of using DICE on state-only distributions is that the operator $B^\pi$ on off-line data $s_T \sim \dt$ requires us to access $s' \sim \cP(\cdot | s_T, \pi(s_T))$, which therefore cannot be solved unless we can access an environment transition model $\cP(\cdot|s,a)$ given arbitrary $(s,a)$.

A potential solution, which does not require learning any forward or inverse model, is to decouple $\pi$ and $Q$ from the min-max objective in \eq{\ref{obj:wdice-state}}, so that they optimizes on different terms:

$D$ optimizes on learning the lower-bound of Wasserstein-1 Distance between $\mupi(s)$ and $\mut(s)$:
\begin{align} \label{obj:wdice-D}
    \max_{||D||_L \leq 1} \cE_{(s) \sim \mut(s)}[D(s)] - \cE_{(s) \sim \mupi} [D(s)]. 
\end{align}

$\pi$ optimizes on minimizing this lower-bound:
\begin{align} \label{obj:wdice-pi}
    \min_{\pi} \cE_{(s) \sim \mupi(s)}[D(s)], 
\end{align}

which means $\pi$ only focus on deriving a distribution of $\mupi$ while not affecting the first term in \eq{\ref{obj:wdice-state}}. This is the practice adopted by GAN and GAIL.

{ \remark \judycom{Needs to verify:}
Given optimal $D$, an optimal $\pi$ to objective function \eq{\ref{obj:wdice-pi}} satisfies $\mupi(s) = \mut(s)$. 
}

After applying changing-of-variables and chain-rule, we reach the following strategy which learns a value-function $v$ and a policy $\pi$ alternatively:

For $v$:
\begin{align*}
   \max_{ ||v||_L \leq 1} \cE_{(s \sim \mut(s)}[(v - B^\pi v) (s))] - \cE_{s_0 \sim p_0  \sim \pi } [ v (s_0) ] 
\end{align*}

For $\pi$:
\begin{align*}
    \max_{ \pi}  \cE_{s_0 \sim p_0  \sim \pi } [ v (s_0) ] 
 \end{align*}

 \judycom{Questions:}
Can we prove that optimizing $v$ and $v$ with separate  objectives still minimizes the Divergence between $\mupi$ and $\mut$ ?


% { \remark \judycom{Needs to verify:}
% Given fixed $\pi$, an optimal $D^*$ to objective \eq{\ref{obj:wdice-D}} satisfies $D(s) = \frac{\mut(s)}{\mupi(s)}$ 
% }




==> supplements/proof_backup.tex <==

\section{Appendix}  
% Based on the assumption, we have the following lemma:
We refer the following lemma from \cite{yang2019imitation} for a coherent presentation:
{\lemma \label{theorem:kl}
%\textbf{Lemma:}
    \begin{align*}
        \KL(\mupi(s,a,s') || \mut(s,a,s')) = \KL(\mupi(s,a) || \mut(s,a)) 
    \end{align*}
}
\begin{proof}
\begin{align*}
    \KL(\mupi(s,a,s') || \mut(s,a,s')) 
    &= \int_{\cS \times \cA \times \cS} \mupi(s,a, s') \log \frac{\mupi(s,a) \cdot \cP(s'|s,a)}{\mut(s,a) \cdot \cP(s'|s,a)} ds da \\
    &=\int_{\cS \times \cA \times \cS} \mupi(s,a, s') \log \frac{\mupi(s,a)}{\mut(s,a)} ds da ds \\
    &= \KL(\mupi(s,a) || \mut(s,a)) 
\end{align*}
\end{proof}


% \subsection{}  \label{appendix:gap-KL}
% %\eq{\ref{eq:gap-KL}}: 
% $$\KL(\mupi(s,a) || \mut(s,a)) = \KL(\mupi(s)||\mut(s)) + \cD_\KL(\pi(a|s)||\pi_E(a|s)).$$

% \begin{proof}
% \begin{align*}
%    \KL(\mupi(s,a) || \mut(s,a)) &= \int_{\cS \times \cA} \mupi(s,a) \log \frac{\mupi(s,a)}{\mut(s,a)} ds da \\
%    &= \int_{\cS \times \cA} \mupi(s,a) \log \frac{\mupi(s) \pi(a|s)}{\mut(s) \pi_E(a|s)} ds da \\ 
%    &= \int_{\cS \times \cA} \mupi(s,a) \big (\log \frac{\mupi(s) }{\mut(s) } + \log \frac{\pi(a|s)}{ \pi_E(a|s)} \big ) ds da \\ 
%    &= \int_{\cS \times \cA} \mupi(s) \log \frac{\mupi(s) }{\mut(s) } ds + \int_{\cS \times \cA} \mupi(s,a) \log \frac{\pi(a|s)}{ \pi_E(a|s)} \big ) ds da \\
%    &= \KL(\mupi(s)||\mut(s)) + \cD_\KL(\pi(a|s)||\pi_E(a|s))
% \end{align*}
% \end{proof}

% A similar equation has been derived by \cite{yang2019imitation}:
% $$\KL(\mupi(s,a) || \mut(s,a)) = \KL(\mupi(s,s')||\mut(s,s')) + \cD_\KL(\mupi(a|s,s')||\pi_E(a|s,s')).$$
% \begin{proof}
% \begin{align*}
%    \KL(\mupi(s,a) || \mut(s,a)) &= \int_{\cS \times \cA \times \cS} \mupi(s,a, s') \log \frac{\mupi(s,a, s')}{\mut(s,a, s')} ds da ds' \\
%    &= \int_{\cS \times \cA \times \cS} \mupi(s,a, s') \log \frac{\mupi(s,s') \mupi(a|s,s')}{\mut(s,s') \mut(a|s,s')} ds da ds'\\ 
%    &= \int_{\cS \times \cA  \times \cS} \mupi(s,a,s') \big (\log \frac{\mupi(s,s') }{\mut(s,s') } + \log \frac{\mupi(a|s,s')}{ \mut(a|s,s')} \big ) ds da ds'\\ 
%    &= \int_{\cS \times \cS} \mupi(s,s') \log \frac{\mupi(s,s') }{\mut(s,s') } ds ds' + \int_{\cS \times \cA \times \cS} \mupi(s,a, s') \log \frac{\mupi(a|s,s')}{ \mut(a|s,s')} \big ) ds da ds'\\
%    &= \KL(\mupi(s,s')||\mut(s,s')) + \cD_\KL(\mupi(a|s,s')||\pi_E(a|s,s'))
% \end{align*}
% \end{proof}

\subsection{} \label{appendix:eq-main}
%\eq{\ref{eq:main}}:
\begin{align*}
    \KL(\mupi(s,s') || \mut(s,s')) \leq \cE_{(s,s')\sim \mupi(s,s')} [\log \frac{\muR(s,s')} {\mut(s,s')}] + \KL[\mupi(s,a) || \muR(s,a)]. 
\end{align*}

\begin{proof}
    \begin{align*}
        \KL(\mupi(s,s') || \mut(s,s'))  &= \int_{\cS \times \cA} \mupi(s,s') \log \frac{\mupi(s,s')}{\mut(s,s')} ds da \\
        &= \int_{\cS \times \cA} \mupi(s,s') \log \Big (\frac{\muR(s,s')} {\mut(s,s')} \cdot \frac{\mupi(s,s')} {\muR(s,s')} \Big )ds da \\
        &= \int_{\cS \times \cA} \mupi(s,s') \log \frac{\muR(s,s')} {\mut(s,s')} ds da + \int_{\cS \times \cA} \mupi(s,s') \log  \frac{\mupi(s,s')} {\muR(s,s')} ds da \\
        &= \cE_{(s,s')\sim \mupi(s,s')} [\log \frac{\muR(s,s')} {\mut(s,s')}] + \KL[\mupi(s,s') || \muR(s,s')]  
    \end{align*}


\end{proof}  

\subsection{} \label{Appendix:lfo-upperbound}
{\assumption{} \label{assume:bounded}
We assume that the density ratios $ \frac{\mupi(s,a)}{\mut(s,a)}$ and $\frac{\mupi(s,a)}{\muE(s,a)}$ are bounded by some finite constant: $$ \exists R_{\text{max}} > 0, \st ~\frac{\mupi(s,a)}{\mut(s,a)} \leq R_{\text{max}}, \frac{\mupi(s,a)}{\muR(s,a)} \leq R_{\text{max}}.$$
}

Based on the above assumption, we have Lemma \ref{lemma:lfo-upperbound}:
\begin{align*}
  \cE_{(s,a)\sim \mupi(s,a)} [\log \frac{\muR(s,a)} {\mut(s,a)}] \leq \cE_{(s, s')\sim \mupi(s, s')}[\log \frac {\muR(s,s')} {\mut(s,s')} ] + C
\end{align*}
%\textbf{Proof of Lemma \ref{lemma:lfo-upperbound}:}

\begin{proof}
\begin{align*}
    &\cE_{(s,a)\sim \mupi(s,a)} [\log \frac{\muR(s,a)} {\mut(s,a)}] = \int_{\cS \times \cA \times \cS } \mupi(s, a) \log \frac {\muR(s,a)} {\mut(s,a)}  ds da \\
    &= \underbrace{\int_{\cS \times \cA \times \cS } \mupi(s, a, s') \log \frac {\muR(s,a, s')} {\mut(s,a, s')}  ds da ds'}_{\text{Lemma \ref{theorem:kl}}}  \\
    &= \int_{\cS \times \cA \times \cS } \mupi(s, a, s') \log \Big ( \frac {\muR(s, s')} {\mut(s,s')} \cdot \frac{\muR(a|s,s')} {\mut(a|s,s')} \Big ) ds da ds' \\
    &= \int_{\cS \times \cA \times \cS } \mupi(s, a, s') \log  \frac {\muR(s, s')} {\mut(s,s')} ds da ds' + \int_{\cS \times \cA \times \cS } \mupi(s, a, s') \log \frac{\muR(a|s,s')} {\mut(a|s,s')}  ds da ds' \\
    %%%%%%
    &= \int_{\cS \times \cA \times \cS } \mupi(s, a, s') \log  \frac {\muR(s, s')} {\mut(s,s')} ds da ds' + \int_{\cS \times \cA \times \cS } \mupi(s, a, s') \Big ( \log \frac{\muR(a|s,s')} {\mupi(a|s,s')}  + \log \frac{\mupi(a|s,s')}{\mut(a|s,s')} \Big) ds da ds' \\
    %%%%
    &= \cE_{(s, s')\sim \mupi(s, s')}[\log \frac {\muR(s,s')} {\mut(s,s')} ]  - \cD_\KL[\mupi(a|s,s') || \muR(a|s,s')] +  \cD_\KL[\mupi(a|s,s') || \mut(a|s,s')\\
    &\leq \cE_{(s, s')\sim \mupi(s, s')}[\log \frac {\muR(s,s')} {\mut(s,s')} ] +  \cD_\KL[\mupi(a|s,s') || \mut(a|s,s')\\
    &= \cE_{(s, s')\sim \mupi(s, s')}[\log \frac {\muR(s,s')} {\mut(s,s')} ] + \underbrace{\KL[\pi(a|s)||\pi_E(a|s)] - \cD_\KL[\mupi(s'|s) || \mut(s'|s)}_{\text{Lemma \ref{lemma:bc-lowerbound-reverse}}}\\
    &\leq \cE_{(s, s')\sim \mupi(s, s')}[\log \frac {\muR(s,s')} {\mut(s,s')} ] +  \KL[\pi(a|s)||\pi_E(a|s)]  \\
    %&\leq \cE_{(s, s')\sim \mupi(s,   s')}[\log \frac {\muR(s,s')} {\mut(s,s')} ]   +  \sup_{\pi } \cD_\KL[\mupi(a|s,s') || \mut(a|s,s')] \\
    &= \cE_{(s, s')\sim \mupi(s,   s')}[\log \frac {\muR(s,s')} {\mut(s,s')} ]   +  C\\
    %%%%%%% 
    \end{align*}
    where $C = \sup_{\pi} \cD_\KL[\mupi(a|s,s') || \mut(a|s,s')]$ is bounded given assumption \ref{assume:bounded}.
\end{proof}

Noted that the last term,  $\sup_{\pi } \cD_\KL[\mupi(a|s,s') || \mut(a|s,s')] $ requires knowlge of expert action labels and therefore cannot be estimated, unless in a deterministic and injective MDP.
  
%  Here, we slightly abuse $\pi_R(a|s)$ to denote:  
%      $$\pi_R(a|s) = \int_{\cS} \muR(a|s,s') ds' = \int_{\cS} \frac{\muR(s,a,s')}{\muR(s,s')} ds' = \frac{\muR(s,a)}{\muR(s)} \leq 1.$$

\textbf{ Remark \ref{lemma:divergence}:} \textit{For distributions $P$ and $Q$, and a convex $f$-function with $f(x)=\frac{1}{2} x^2$, we have
\begin{align*}
    \cD_\KL[P||Q] \leq \cD_f[P||Q]. 
\end{align*} 
\vskip -0.1in
}
\begin{proof}

Given two distributions $P$ and $Q$, define their density ratio as $w_{p|q}= \frac{p(x)}{q(x)} \geq 0$. 
%
If we consdier a function $g(w)= w \log(w) - \frac{1}{2} w^2$, $g(w)$ is constantly decreasing when $w \in (0, \infty)$, as $\frac{\partial g} {\partial w}=\log w+ 1 - w \leq 0 ~\forall w \geq 0$.

Since KL-Divergence is a special case of $f$-divergence with $f_{\KL}(x)=x \log x$, it is sufficient to show that:
\begin{align*}
    \cD_{\KL}[P||Q] - \cD_f[P||Q]  &= \int_\cX q(x)  \Big (w_{p/q} \log(w_{p/q}) - \frac{1}{2} (w_{p/q})^2 \Big ) dx \\
    &\leq \int_\cX q(x) \sup_{w \in (0,+\infty)} (w \log(w) - \frac{1}{2} w^2 ) dx \\
    &= \int_\cX q(x) \lim_{w \to 0^+} (w \log(w) - \frac{1}{2} w^2 ) dx \\
    &= 0.
\end{align*}
\end{proof}

\subsection{Inverse Model Constraints} \label{appendix:inverse-proof} 
%  

{\assumption \label{assume:mdp}
    We assume the MDP is deterministic: 
    %$$\cP(s'|s,a)=\delta(s' - g(s,a)),$$ 
    %$\delta$ a Dirac delta function,  
    $$\exists g:\cS \times \cA \to \cS \text{ a deterministic function, }  \st ~\cP(s'|s,a) = 0~\forall s' \neq g(s,a).$$
}  

{\assumption \label{assume:support}
We assume that the support of expert transition distribution $\mut(s,s')$ is covered by $\muR(s,s')$: 
    $$\mut(s,s') > 0 \Longrightarrow \muR(s,s') > 0.$$
}


{\remark \label{remark:optimal-inverse}
Given arbitrary policy $\pi$, and a policy $\bpi$, $\st ~\bpi(a|s) \propto \muR(a|s,s') ~\forall (s,s') \sim \mut(s,s')$,
$$ \cD_\KL[\mut(s'|s)||\mupi(s'|s)] \geq \cD_\KL[\mut(s'|s)||\mu^\bpi(s'|s)].$$
}
We provide proof in a tabular case:
\begin{proof}
    \begin{align*}
        &\cD_\KL[\mut(s'|s)||\mu^\bpi(s'|s)] \\
        &= \cE_{(s,s') \sim \mut(s,s') } \big[  \log \frac{\mut(s'|s)}{\mu^\bpi(s'|s)} \big] \\
        &= \underbrace{ \cE_{(s,s')\sim \mut(s,s') } [\log \mut(s'|s)] }_{\text{fixed } \wrt \pi}- \cE_{(s,s')\sim \mut(s,s') }\log \mu^\bpi(s'|s) \\
        &= H(\mut(s'|s))  - \cE_{(s,s') \sim \mut(s,s')}\big[ \log \cE_{a\sim\bpi(\cdot|s)} [\cP(s'|s,a)] \big]\\ 
        &= H(\mut(s'|s))  - \underbrace{\cE_{(s,s') \sim \mut(s,s')}\big[ \log \cE_{a\sim\bpi(\cdot|s)} [1] \big]}_{\text{Assumption \ref{assume:mdp}}}\\ 
        &= H(\mut(s'|s)). \\ 
    \end{align*}
    Noted that given Assumption \ref{assume:support}, $\forall (s,s') \sim \mut(s,s'),$  $\muR(s,s')  > 0$. Combine with Assumption \ref{assume:mdp}: $$\forall (s,s') \sim \mut(s,s'), \bpi(a|s) > 0 \Longrightarrow \muR(a|s,s') > 0 \Longrightarrow \cP(a|s,s') = 1.$$

    At the meantime:
    \begin{align*}
        &\cD_\KL[\mut(s'|s)||\mupi(s'|s)] \\
        &= H(\mut(s'|s))  - \cE_{(s,s') \sim \mut(s,s')}\big[ \log \cE_{a\sim\pi(\cdot|s)} [\cP(s'|s,a)] \big]\\ 
        &\leq H(\mut(s'|s))  - \cE_{(s,s') \sim \mut(s,s')}\big[ \log \cE_{a\sim\pi(\cdot|s)} [1] \big]\\ 
        &= H(\mut(s'|s)).\\ 
    \end{align*}

    Based on the above we conclude:
    $$\cD_\KL[\mut(s'|s)||\mu^\bpi(s'|s)] \leq \cD_\KL[\mut(s'|s)||\mupi(s'|s)].$$
\end{proof}
% {\remark \label{remark:optimal-inverse}
% For arbitrary policy $\pi$, and for any off-policy distribution $\muR$ which satisfies Assumption \ref{assume:support}, we have the following property:
% \begin{small}
%    \begin{align*}
%     %\cE_{(s,s') \sim \mut(s,s')}\Big[ \log \Big( \pi(a|s) \cP(s'|s,a) \Big) \Big]  \leq \cE_{(s,s') \sim \mut(s,s')}\Big[ \log \Big(\muR(a|s,s') \cP(s'|s,a) \Big)\Big]
%     \cE_{(s,s') \sim \mut(s,s')} \cE_{a \sim \pi(\cdot|s)}[\cP(s'|s,a)] \leq  \cE_{a \sim \muR(\cdot|s,s')}[\cP(s'|s,a)].
%     %= \int_{\cA \times \cS \times \cS} \mut(s,s') \log \pi(a|s) \cP(s'|s,a) da ds' ds  \leq \int_{\cA \times \cS \times \cS } \muR(a|s,s') \cP(s'|s,a) da ds' ds.
%    \end{align*}
% \end{small}
% }

% We provide proof in a tabular setting.
% \begin{proof}
% Based on Assumption \ref{assume:mdp}, for arbitrary $\muR$, we have:
% \begin{align}
%     %\forall &(s,s') \sim \mut(s,s'), \nonumber\\
%     \muR(a|s,s') > 0 \Longrightarrow \muR(s,a)\cP(s'|s,a) > 0 \Longrightarrow  \cP(s'|s,a) = 1, \label{backward}
% \end{align}

% which leads to the following:
% \begin{align*}
%    % &\cE_{s' \sim \mut(s'|s)}\Big[   \muR(a|s,s') \cP(s'|s,a)  \Big] \\
%   %& \int_{\cA} \muR(a|s,s') \cP(s'|s,a) da  \\
%   %= & \int_{a \sim \cA, g(s,a)=s'} \muR(a|s,s') \delta(0) da + \int_{a \sim \cA, g(s,a) \neq s'} \muR(a|s,s') \delta(s' - g(s,a)) da \\
% %   = & \int_{\cA } \underbrace{\muR(a|s,s')\delta(0) da }_\text{\eq{\ref{backward}}} \\
% %   = & \delta(0)
% \forall (s,s') \sim \muR(s,s'), \cE_{a \sim \muR(\cdot|s,s')} [\cP(s'|s,a)] = \cE_{a \sim \muR(\cdot|s,s')}[1] = 1.
% \end{align*}
% %
% On the other hand:
% \begin{align*}
%     % \forall (s,s') \sim \mut(s,s'), & \int_{a \sim \cA} \pi(a|s) \cP(s'|s,a) da \\
%     % = & \int_{a \sim \cA} \pi(a|s) \delta(s' - g(s,a)) da \\
%     % \leq & \int_{a \sim \cA} \pi(a|s) \delta(0) da\\
%     % = & \delta(0) 
%     \forall (s,s') \sim \muR(s,s'), \cE_{a \sim \pi(\cdot|s)} [\cP(s'|s,a)] \leq \cE_{a \sim \muR(\cdot|s,s')}[1] = 1.
% \end{align*}
% Combining above leads to:
% $$\forall (s,s') \sim \muR(s,s'), \cE_{a \sim \pi(\cdot|s)}[\cP(s'|s,a)] \leq  \cE_{a \sim \muR(\cdot|s,s')}[\cP(s'|s,a)]. $$
% Based on Assumption \ref{assume:support}:
% $$\cE_{(s,s') \sim \mut(s,s')} \Big[\cE_{a \sim \pi(\cdot|s)}[\cP(s'|s,a)] \Big]\leq  \cE_{a \sim \muR(\cdot|s,s')}[\cP(s'|s,a)]$$ 
% \end{proof}

% \textbf{Remark \ref{remark:inverse-constraint}:}
% $$\pi(\cdot|s) \propto \PI^*(\cdot|s,s'), \forall (s, s') \sim \mut(s,s') \Longrightarrow \pi = \arg \min_\pi \cD_\KL[\mut(s'|s) || \mupi(s'|s)].$$
% \begin{proof}
% Assume that we have learn an optimal inveres model with $\PI^*=\muR(a|s,s)$, it naturally holds that:
% \begin{align} \label{eq:inverse}
%     \forall (s,s') \sim \mut(s,s'), \underbrace{\int_{\cA} \pi(a|s) \cP(s'|s,a) da  \leq \int_{\cA} \PI^*(a|s,s') \cP(s'|s,a)}_\text{Lemma \ref{remark:optimal-inverse}} da. 
% \end{align} 

% Let us define the \textit{forward state-transition distribution} induced by $\pi$ as $\mupi(s’|s)$: $$\mupi(s’|s)= \int_\cA \pi(a|s) \cP(s'|s,a) da,$$ and the same for $\mut(s’|s)$.
% %
% Now consider the \textit{conditional} $\KL$-divergence between $\mut(s'|s)$ and $\mupi(s'|s)$:
% \begin{align*}
%     %\arg \min_\pi
%     &- \cD_\KL[\mut(s'|s) || \mupi(s'|s)] := - \int_{\cS \times   \cS} \mut(s) \mut(s'|s) \log \frac{\mut(s’|s) }{\mupi(s’|s) } ds' ds \\
%     &= - \int_{\cS \times   \cS} \mut(s) \mut(s'|s) \log  \mut(s’|s) ds ds' + \int_{\cS \times   \cS} \mut(s) \mut(s'|s) \log  \mupi(s’|s) ds' ds  \\
%     &= \underbrace{H(\mut(s'|s))}_{\text{not optimizable~} \wrt \pi} + \int_{\cS \times   \cS} \mut(s) \mut(s'|s)  \log  \mupi(s’|s) ds' ds \\
%     &= H(\mut(s'|s))   +  \lkxcom{\max_{\pi}} \int_{\cS \times   \cS} \mut(s,s')  \log  \int_{\cA} \pi(a|s) \cP(s'|s,a) da ds' ds \\
%     &\lkxcom{=} H(\mut(s'|s))   +  \int_{\cS \times   \cS} \mut(s,s')   \int_{\cA}  \underbrace{   \PI^*(a|s,s') \cP(s'|s,a) }_{\text{ \eq{ \ref{eq:inverse} }}}   da ds' ds. \\
% \end{align*} 

% \vskip -0.1 in
% $\cD_\KL[\mut(s'|s) || \mupi(s'|s)] $ is minimized when $\pi$ follows $\PI^*(\cdot|s,s')$: $$\pi(\cdot|s) \propto \PI^*(\cdot|s,s') ~ \forall s, s \sim \mut(s,s').$$ 
% \end{proof}
% Intuitively, this constraint encourages \textit{mode-covering}, by leading policy to take actions that \textit{cover} the ideal next state. Since $\PI^*(\cdot|s,s')$ only has \textit{support} on actions that yields transition $s \to s'$, following this constraint can avoid policy from deviating to other states. 

{\lemma \label{lemma:bc-lowerbound-reverse}:
    \begin{align*}
        \cD_\KL[\pi(a|s)||\pi_E(a|s)] = \cD_\KL[\mupi(s'|s)||\mut(s'|s)] +  \cD_\KL[\mupi(a|s,s')||\mut(a|s,s')].  
    \end{align*}
}  
\begin{proof}
    Based on the definition of $\mupi(a|s,s')$: 
    \begin{align} \label{eq:invese-def}
        \mupi(a|s,s')= \frac{\pi(a|s) \cP(s'|s,a)}{\int_\cA \pi(\ba|s) \cP(s'|s,\ba)d\ba} = \frac{\pi(a|s) \cP(s'|s,a)}{\mupi(s'|s)},    
    \end{align}
    and similar for $\mut(a|s,s')$, we can derive:
    \begin{align*}
        &\cD_\KL[\pi(a|s) || \pi_E(a|s)] \\
        = & \int_{\cS \times \cA} \mupi(s,a)  \log \frac{\pi(a|s)} {\pi_E(a|s)} da ds \\
        = & \int_{\cS \times \cA \times \cS} \mupi(s,a)  \log \frac{\pi(a|s)} {\pi_E(a|s)} ds' da ds\\
        = & \int_{\cS \times \cA \times \cS} \mupi(s,a,s') \log \frac{\pi(a|s) \cP(s'|s,a)  } {\pi_E(a|s) \cP(s'|s,a) } ds'da ds \\
        = & \int_{\cS \times \cA \times \cS} \mupi(s,a,s') \underbrace{\log \frac {\mupi(a|s,s') \mupi(s'|s) }{ \mut(a|s,s') \mut(s'|s) }} _{\text{ \eq{\ref{eq:invese-def}}}} ds'da ds \\
        = & \int_{\cS \times \cA \times \cS} \mupi(s,a,s') \Big( \log \frac{ \mupi(a|s,s')  } {\mut(a|s,s') } + \log \frac{\mupi(s'|s)}{\mut(s'|s)} \Big) ds' da ds \\
        = & \int_{\cS \times \cA \times \cS} \mupi(s,a,s')  \log \frac{ \mupi(a|s,s')  } {\mut(a|s,s') } ds' da ds + \int_{\cS \times \cA \times \cS} \mupi(s,a,s') \log \frac{ \mupi(s'|s)  } {\mut(s'|s) } ds' da ds \\
        = & \cD_\KL[\mupi(a|s,s') || \mut(a|s,s')] +  \cD_\KL[\mupi(s'|s)||\mut(s'|s)].
    \end{align*}
\end{proof}

\textbf{Lemma \ref{lemma:bc-lowerbound}:}  
    \begin{align*}
        \cD_\KL[\pi_E(a|s)||\pi(a|s)] = \cD_\KL[\mut(s'|s)||\mupi(s'|s)] +  \cD_\KL[\mut(a|s,s')||\mupi(a|s,s')].  
    \end{align*}
Proof is same as Lemma \ref{lemma:bc-lowerbound-reverse} by switching $\pi$ with $\pi_E$.
% \begin{proof}
%     Based on the definition of $\mupi(a|s,s')$: 
%     \begin{align} \label{eq:invese-def}
%         \mupi(a|s,s')= \frac{\pi(a|s) \cP(s'|s,a)}{\int_\cA \pi(\ba|s) \cP(s'|s,\ba)d\ba} = \frac{\pi(a|s) \cP(s'|s,a)}{\mupi(s'|s)},    
%     \end{align}
%     and similar for $\mut(a|s,s')$, we can derive:
%     \begin{align*}
%         &\cD_\KL[\pi_E(a|s) || \pi(a|s)] \\
%         = & \int_{\cS \times \cA} \mut(s,a)  \log \frac{\pi_E(a|s)} {\pi(a|s)} da ds \\
%         = & \int_{\cS \times \cA \times \cS} \mut(s,a)  \log \frac{\pi_E(a|s)} {\pi(a|s)} ds' da ds\\
%         = & \int_{\cS \times \cA \times \cS} \mut(s,a,s') \log \frac{\pi_E(a|s) \cP(s'|s,a)  } {\pi(a|s) \cP(s'|s,a) } ds'da ds \\
%         = & \int_{\cS \times \cA \times \cS} \mut(s,a,s') \underbrace{\log \frac{ \mut(a|s,s') \mut(s'|s) } {\mupi(a|s,s') \mupi(s'|s) }}_{\text{ \eq{\ref{eq:invese-def}}}} ds'da ds \\
%         = & \int_{\cS \times \cA \times \cS} \mut(s,a,s') \Big( \log \frac{ \mut(a|s,s')  } {\mupi(a|s,s') } + \log \frac{\mut(s'|s)}{\mupi(s'|s)} \Big) ds' da ds \\
%         = & \int_{\cS \times \cA \times \cS} \mut(s,a,s')  \log \frac{ \mut(a|s,s')  } {\mupi(a|s,s') } ds' da ds + \int_{\cS \times \cA \times \cS} \mut(s,a,s') \log \frac{ \mut(s'|s)  } {\mupi(s'|s) } ds' da ds \\
%         = & \cD_\KL[\mut(a|s,s') || \mupi(a|s,s')] +  \cD_\KL[\mut(s'|s)||\mupi(s'|s)].
%     \end{align*}

% \end{proof}
%while the main objective works by encouraging \textit{mode seeking}.

%Operator $\cB^\pi$ depends on a synthetic reward from discriminator, optimized by \eq{\ref{eq:offpolicy-d}}. 
\subsection{ Derivation of \eq{\ref{obj:main-dice}}:} \label{Appendix:obj:main-dice}
\begin{align*} %\label{obj:main-dice-prove}
    %\JOPOLO(\pi, Q) &=  \cE_{(s, a, s')\sim \mupi(s, a, s')}[ r(s,s') - (\cB^\pi Q - Q)(s,a)] + \alpha E_{(s,a) \sim \muR}[f_*(\frac{1}{\alpha}(\cB^\pi Q - Q)(s,a))]  
    \JOPOLO(\pi, Q) &=  \cE_{(s, a, s')\sim \mupi(s, a, s')}[ r(s,s') - (\cB^\pi Q - Q)(s,a)] +  E_{(s,a) \sim \muR}[f_*((\cB^\pi Q - Q)(s,a))],  
\end{align*}
where $\cB^\pi Q(s,a)= \cE_{s'\sim P(\cdot|s,a),a' \sim \pi(\cdot|s')}\Big [r(s,s') + \gamma Q(s',a') \Big].$ 
\begin{proof}
    The first term in the RHS can be reduced to the following:
\begin{align*} 
   &\cE_{(s, a, s')\sim \mupi(s, a, s')}[ r(s,s') - (\cB^\pi Q - Q)(s,a)]  \\
   = &\cE_{(s, a)\sim \mupi(s, a)}\Big[ \cE_{s' \sim \cP(\cdot|s,a)} [r(s,s') ]- \cE_{s' \sim \cP(\cdot|s,a)} [(\cB^\pi Q - Q)(s,a)] \Big]  \\
   = &\cE_{(s, a)\sim \mupi(s, a)}\Big[ \cE_{s' \sim \cP(\cdot|s,a)} [r(s,s') ] + Q(s,a) - \cE_{s' \sim \cP(\cdot|s,a)} [\cB^\pi Q (s,a)] \Big]  \\
   = &\cE_{(s, a)\sim \mupi(s, a)}\Big[ \cE_{s' \sim \cP(\cdot|s,a)} [r(s,s') ] + Q(s,a) - \cE_{s' \sim \cP(\cdot|s,a), a' \sim \pi(\cdot|s')} [ r(s,s') + \gamma  Q (s',a')] \Big]  \\
   = &\cE_{(s, a)\sim \mupi(s, a)}[Q(s,a)- \gamma \cE_{s' \sim \cP(\cdot|s,a), a' \sim \pi(\cdot|s')} [Q(s',a' )] ] \\
   = & (1-\gamma)\sum_{t=0}^{\infty} \gamma^t \cE_{s \sim \mu^\pi_t, a \sim \pi(s)}[Q(s,a)] - (1-\gamma)\sum_{t=0}^{\infty} \gamma^{t+1} \cE_{s \sim \mu^\pi_t, a \sim \pi(\cdot|s),s' \sim \cP(\cdot|s,a), a' \sim \pi(\cdot|s')} [Q(s',a' )] ]  \\
   = & (1-\gamma)\sum_{t=0}^{\infty} \gamma^t \cE_{s \sim \mu^\pi_t, a \sim \pi(s)}[Q(s,a)] - (1-\gamma)\sum_{t=0}^{\infty} \gamma^{t+1} \cE_{s \sim \mu^\pi_{t+1}, a \sim \pi(\cdot|s) } [Q(s,a)] ]  \\
   = & (1-\gamma) \cE_{s\sim p_0, a_0 \sim \pi(\cdot|s_0)}[Q(s_0,a_0)]
\end{align*}
Therefore:
%$$\JOPOLO(\pi, Q) = (1-\gamma) \cE_{s\sim p_0, a_0 \sim \pi(s_0)}[Q(s_0,a_0)] + \alpha E_{(s,a) \sim \muR}[f_*(\frac{1}{\alpha}(\cB^\pi Q - Q)(s,a))].$$ 
$$\JOPOLO(\pi, Q) = (1-\gamma) \cE_{s\sim p_0, a_0 \sim \pi(\cdot|s_0)}[Q(s_0,a_0)] +  E_{(s,a) \sim \muR}[f_*((\cB^\pi Q - Q)(s,a))].$$ 
\end{proof}
